A Numerical Investigation of Extremum-Seeking-Based Command Generation for Adaptively Controlled Systems

We develop an adaptive feedback control technique that combines an extremum-seeking-based command generator (ECG) with indirect adaptive control. In particular, ECG is used to generate commands that asymptotically optimize a cost function that is measured but whose functional form is unknown. For feedback control with command following and stabilization, the present paper combines ECG with predictive cost adaptive control (PCAC), which is an indirect adaptive control extension of model predictive control (MPC). PCAC extends generalized predictive control (GPC) by using quadratic programming to enforce output constraints and recursive least squares (RLS) with variable-rate forgetting (VRF) for system identification. The resulting ECG/PCAC framework combines command generation with closed-loop system identification and online optimization. The contribution of this paper is a numerical investigation of ECG/PCAC for adaptive stabilization, command following, and disturbance rejection

==> Figures/ESPCAC.tex <==
\resizebox{\textwidth}{!}{%
\begin{tikzpicture}[>={stealth'}, line width = 0.5mm]
%
\node[draw = none] at (0,0) (orig) {};
%
\node[smallblock, fill=green!20,rounded corners, minimum height = 18em, minimum width = 25em] at ([yshift = -4.5em]orig.center) (PCAC){};
%
\node[above] at (PCAC.north) {\bf \large$\begin{array}{c} \mbox{Predictive Cost Adaptive Control} \end{array}$};
%
\node[smallblock, rounded corners, minimum height = 5em, minimum width = 20em] at (orig.center) (MPC) {$\begin{array}{c} \mbox{\bf\large Model Predictive Control} \\ \mbox{QP for output feedback} \\ \mbox{with control and output constraints} \end{array}$};
%
\node[smallblock, rounded corners, minimum height = 5em, minimum width = 20em] at ([yshift = -9em]MPC.center) (RLSID) {$\begin{array}{c} \mbox{\bf\large Online System Identification} \\ \mbox{RLS/VRF for online identification} \\ \mbox{with variable-rate forgetting} \end{array}$};
%
\node[smallblock, fill=red!20, rounded corners, minimum height = 7em, minimum width = 17em] at ([xshift = 30em]MPC.center) (system) {$\begin{array}{c} \mbox{\bf\large System Dynamics} \\ \mbox{Mass-Spring System} \end{array}$};
%
\node[smallblock, fill=yellow!20, rounded corners, minimum height = 7em, minimum width = 10em] at ([xshift = 25em]system.center) (costfn) {$\begin{array}{c} \mbox{\bf\large Cost Function} \\ \mbox{$J = f(y)$} \end{array}$};
%
\node[smallblock, fill=magenta!20, rounded corners, minimum height = 7em, minimum width = 17em] at ([yshift = -25em]system.center) (ESC) {$\begin{array}{c} \mbox{\bf\large Extremum-Seeking Control} \\ \mbox{$\textcolor{red}{TODO}$} \end{array}$};
%
\draw[->] (system.east) -- ([xshift = 7em]system.east) |- ([yshift = -1em]RLSID.east);
%
\draw[->] (system.east) -- node[above] {\bf \large Measurement $y_k$}(costfn.west);
%
\draw[->] (system.east) -- ([xshift = 7em]system.east) |- node[above, near end] {\bf \large Measurement $y_k$} ([xshift = -4em, yshift = -7.5em]RLSID.west) |- ([yshift=-1em]MPC.west);
%
\draw[->] ([xshift = -8em]RLSID.north) -- node[xshift = 9.8em] {\bf \large  Estimated Model Coefficients $\theta_k$} ([xshift = -8em]MPC.south);
%
\draw[->] (MPC.east) -- node[above, xshift = 1.25em] {\bf \large Control $u_k$} (system.west);
%
\draw[->] (MPC.east) -- ([xshift = 7em]MPC.east) |- ([yshift = 1em]RLSID.east);
%
\draw[->] ([xshift = -5.25em, yshift = 3em]system.north) -- node[xshift = 5.1em] {\bf \large Disturbance $w_k$} ([xshift = -5.25em]system.north);
%
\draw[->] (costfn.east) -- ([xshift = 1em]costfn.east) |- node[above, near end] {\bf \large Cost Measurement $J_k$} (ESC.east);
%
\draw[->] (ESC.west) -- node[above, near start] {\bf \large Command $r_k$} ([xshift = -37em]ESC.west)  |-  ([yshift = 1em]MPC.west);
%
\end{tikzpicture}
}

==> PCAC_review.tex <==
% As developed in \cite{islamPCAC}, 
% PCAC is an extension of model predictive control (MPC)
% %
% \cite{kwon2006receding,camacho2013model,cairano2018MPC,eren2017model}
% %
% based on indirect adaptive control. 
% %
% Unlike data-driven MPC \cite{allgowerlearning2022}, PCAC uses no data record or prior model, either analytical or empirical.
% %
% Instead, PCAC uses online, closed-loop system identification based on recursive least squares (RLS) with variable-rate forgetting \cite{islam2019recursive,adamRLS2020,ankitRLS2020,bruceNandSRLS,mohseni2022recursive}.
% %
% PCAC relies on self-generated persistency for system identification \cite{islamPCAC} and does not use probing as in dual control \cite{mesbahMPCdual2}.
% %
% PCAC has been applied to 
% %
% noise and vibration control \cite{rezaMSSP,PCACRijkeACC2025,rileyBACT2024},
% %
% atmospheric flight control \cite{rileyQCACC2025,rileyScitech2025}, 
% %
% and flow control \cite{PCACAirfoilACC2024};
% %
% \cite{rezaMSSP,PCACRijkeACC2025,rileyQCACC2025} include experimental investigations. 
% %
% Figure \ref{PCACBlock} shows how PCAC combines online identification with output-feedback MPC. 
% %






% PCAC is an extension of generalized predictive control (GPC) \cite{ClarkeGPC1,ClarkeGPC2,Bitmead:90,Mosca:95}.
% %
% In particular, PCAC uses quadratic programming to enforce output constraints in MPC, and uses RLS with VRF to accelerate learning when the dynamics of the controlled system change.
% %
% A major benefit of PCAC derived from MPC is the ability to constrain the requested actuator inputs.
% %
% This ability includes both magnitude and rate saturation, which can be specified and enforced within the QP optimization.
% %
% This feature allows the user to respect realistic hardware constraints and limit excessive actuator activity.








% \begin{figure*}[htbp!]
% \centering
% \resizebox{\textwidth}{!}{%
% %
% \begin{tikzpicture}[>={stealth'}, line width = 0.5mm]
% %
% \node[draw = none] at (0,0) (orig) {};
% %
% \node[smallblock, fill=green!20,rounded corners, minimum height = 18em, minimum width = 25em] at ([yshift = -4.5em]orig.center) (PCAC){};
% %
% \node[above] at (PCAC.north) {\bf \large$\begin{array}{c} \mbox{Predictive Cost Adaptive Control} \end{array}$};
% %
% \node[smallblock, rounded corners, minimum height = 5em, minimum width = 20em] at (orig.center) (MPC) {$\begin{array}{c} \mbox{\bf\large Model Predictive Control} \\ \mbox{QP for output feedback} \\ \mbox{with control and output constraints} \end{array}$};
% %
% \node[smallblock, rounded corners, minimum height = 5em, minimum width = 20em] at ([yshift = -9em]MPC.center) (RLSID) {$\begin{array}{c} \mbox{\bf\large Online System Identification} \\ \mbox{RLS/VRF for online identification} \\ \mbox{with variable-rate forgetting} \end{array}$};
% %
% \node[smallblock, fill=red!20, rounded corners, minimum height = 7em, minimum width = 17em] at ([xshift = 30em]MPC.center) (system) {$\begin{array}{c} \mbox{\bf\large System Dynamics} \\ \mbox{Mass-Spring System} \end{array}$};
% %
% \draw[->] (system.east) -- ([xshift = 1em]system.east) |- ([yshift = -1em]RLSID.east);
% %
% \draw[->] (system.east) -- ([xshift = 1em]system.east) |- node[above, near end] {\bf \large Measurement $y_k$} ([xshift = -5em, yshift = -7.5em]RLSID.west) |- ([yshift=-1em]MPC.west);
% %
% \draw[->] ([xshift = -8em]RLSID.north) -- node[xshift = 9.8em] {\bf \large  Estimated Model Coefficients $\theta_k$} ([xshift = -8em]MPC.south);
% %
% \draw[->] (MPC.east) -- node[above, xshift = 1.25em] {\bf \large Control $u_k$} (system.west);
% %
% \draw[->] (MPC.east) -- ([xshift = 7em]MPC.east) |- ([yshift = 1em]RLSID.east);
% %
% \draw[->] ([xshift = -12em, yshift = 1em]MPC.west) -- node[above, xshift = -1.5em] {\bf \large Command $r_k$} ([yshift = 1em]MPC.west);
% %
% \draw[->] ([xshift = -5.25em, yshift = 3em]system.north) -- node[xshift = 5.1em] {\bf \large Disturbance $w_k$} ([xshift = -5.25em]system.north);
% %
% \end{tikzpicture}
% }
% %
% \caption{PCAC block diagram.  
% %
% The online, closed-loop system identification is based on recursive least squares (RLS) with variable-rate forgetting (VRF). The model predictive control (MPC) algorithm, which is based on quadratic programming (QP), uses the estimated model coefficients ${{\theta}}_k$ to create a predictive function model, which is used by QP to determine the control input ${u}_k$ subject to control and output constraints. 
% } \label{PCACBlock}
% %
% \end{figure*}





==> PackagesCommands.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%% PACKAGES %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{amsmath} % assumes amsmath package installed
% \usepackage{amssymb}  % assumes amsmath package installed
\usepackage{amsfonts}
\usepackage{amsthm}

\newtheorem{theorem}{Theorem}
\newtheorem{assumption}{Assumption}
\newtheorem{proposition}{Proposition}[section]
\theoremstyle{definition}
\newtheorem{definition}{Definition}[section]
% % \newtheorem{definitionSec}{Definition}[subsection]
\newtheorem{exmp}{Example}[section]
% \newtheorem{exmpSec}{Example}[subsection]
\newtheorem{fact}{Fact}[section]
% \newtheorem{proposition}{Proposition}[section]
% \newtheorem{factSec}{Fact}[subsection]
% \newtheorem{theorem}{Theorem}[section]
\newtheorem{problem}{Problem}[section]
\newtheorem{remark}{Remark}
\newtheorem{lemma}{Lemma}[section]


% \newtheorem{prob}{Problem}[section]
\newtheorem{prob}{Problem}

% \usepackage{graphicx}
% \usepackage{epsfig}
% \usepackage{epstopdf}
% \usepackage{math tools}
% \usepackage{color}
% \usepackage[utf8]{inputenc}
%\pagestyle{plain}

% \usepackage{subfigure}
% \usepackage{subfig}
\usepackage{float} 
\usepackage[skip=0em,font=footnotesize]{caption}
% \usepackage{wrapfig}%   wrap figures/tables in text (i.e., Di Vinci style)
% \usepackage[export]{adjustbox}

% \usepackage{geometry}
% \usepackage{indentfirst}


% \usepackage{epsfig} % for postscript graphics files

% \usepackage{lastpage}
% \usepackage{fancyhdr}
% \pagestyle{fancy} 
% \cfoot{\thepage\ of \pageref{LastPage}}
% \fancyhead{}
% \renewcommand{\headrulewidth}{0pt}

% \usepackage{mathptmx} % assumes new font selection scheme installed
% \usepackage{times} % assumes new font selection scheme installed


% \usepackage[mathscr]{euscript}

% \usepackage{newtxtext}
% \usepackage{newtxmath}

% \usepackage{subfiles}
% \usepackage{cancel}
% \usepackage{imakeidx}

%\usepackage{citesort}
%\usepackage[fleqn]{amsmath}
%\usepackage{fullpage}
%\usepackage[top=0.75in,bottom= 0.75in,left = 0.75in, right = 0.75in]{geometry}
\usepackage[margin = 1in]{geometry}

%\parskip = -0.5pt
%\parindent = 2pt %0in


%\usepackage{multicol}
%\usepackage{caption}
%\usepackage[skip=2pt]{caption}
%\usepackage[skip=1pt,font=footnotesize]{caption}
%\usepackage[skip=1pt,font=small]{caption}
%\usepackage{subcaption}






\usepackage{tikz}
\usetikzlibrary{shapes,arrows,calc,positioning}
\tikzstyle{bigblock} = [draw, fill=blue!20, rectangle, 
    minimum height=6em, minimum width=8em]
\tikzstyle{medblock} = [draw, fill=blue!20, rectangle, 
    minimum height=4em, minimum width=4em]    
\tikzstyle{mux} = [draw, fill=black!20, rectangle, 
    minimum height=5em, minimum width=0.1em]    
\tikzstyle{smallblock} = [draw, fill=blue!20, rectangle, 
    minimum height=2em, minimum width=3em]
    
\tikzstyle{data_block} = [draw, fill=green!20, rectangle, 
    minimum height=2em, minimum width=3em]
\tikzstyle{ops_block} = [draw, fill=blue!20, rectangle, 
    minimum height=2em, minimum width=3em]    
\tikzstyle{est_block} = [draw, fill=red!20, rectangle, 
    minimum height=2em, minimum width=3em]    
    
\tikzstyle{sum} = [draw, fill=blue!20, circle, node distance=1cm,minimum height=0.5cm]
\tikzstyle{signal} = [coordinate]
\tikzstyle{pinstyle} = [pin edge={to-,thin,black}]
\tikzstyle{block} = [draw, fill=blue!20, rectangle, 
    minimum height=3em, minimum width=9em]
\tikzstyle{blockS} = [draw, fill=blue!20, rectangle, 
    minimum height=3em, minimum width=4em]    
\tikzstyle{input} = [coordinate]
\tikzstyle{output} = [coordinate]
\usetikzlibrary{matrix}

\usetikzlibrary{positioning}
\usetikzlibrary{math} 



\usepackage{hyperref}
\usepackage{xcolor}
\hypersetup{
    colorlinks,
    linkcolor={blue!100!black},
    citecolor={blue!50!black},
    urlcolor={blue!80!black}
}

% \usepackage{diagbox}


%\newtheorem{definition}{Definition}[section]
%\usepackage{biblatex}
% \addbibresource{mendeley_v2.bib}

% \usepackage[square, numbers, sort&compress]{natbib} 
% \setcitestyle{square braces, numbers}
%\usepackage{cite}



%\usepackage[nomarkers,figuresonly]{endfloat}

% \renewcommand{\familydefault}{\rmdefault}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%% COMMANDS %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\bc}{\begin{center}}
\newcommand{\ec}{\end{center}}
\newcommand{\benum}{\begin{enumerate}}
\newcommand{\eenum}{\end{enumerate}}
\newcommand{\nn}{\nonumber}
\newcommand{\matl}{\left[ \begin{array}}
\newcommand{\matr}{\end{array} \right]}

\renewcommand{\matl}{\begin{bmatrix}}
\renewcommand{\matr}{\end{bmatrix}}

\newcommand{\matls}{\left[ \begin{smallmatrix}}
\newcommand{\matrs}{\end{smallmatrix} \right]}
\newcommand{\isdef}{\stackrel{\triangle}{=}}
\newcommand{\pr}[1]{{#1}^{\prime}}
\newcommand{\inv}{^{-1}}
\newcommand{\row}[1]{{\rm row}_{#1}}
\newcommand{\col}[1]{{\rm col}_{#1}}
\newcommand{\arrowup}[1]{\stackrel{#1}{\SLeftarrow}}
\newcommand{\smin}{\stackrel{\min}{\sim}}
\newcommand{\jw}{\jmath \omega}
\newcommand{\omegan}{\omega_{\rm n}}
\newcommand{\omegad}{\omega_{\rm d}}
\newcommand{\omegar}{\omega_{\rm r}}
\newcommand{\omegani}{\omega_{{\rm n}i}}
\newcommand{\omegans}[1]{\omega_{{\rm n}_{#1}}}
\newcommand{\MSig}{{\mit\Sigma}}
\newcommand{\half}{\tfrac{1}{2}}
\newcommand{\vect}[1]{\overset{\rightharpoonup}{#1}}
\newcommand{\HS}{\hat S}
\newcommand{\HI}{\hat I}
\newcommand{\rmThat}{{\hat{\rm T}}}
\newcommand{\asthat}{{\hat*}}
\newcommand{\dpder}[2]{\displaystyle\frac{\partial {#1}}{\partial {#2}}}
\newcommand{\der}[2]{\mbox{$\frac{d{#1}}{d{#2}}$}}
\newcommand{\dder}[2]{\displaystyle{\frac{d{#1}}{d{#2}}}}
\newcommand{\pder}[2]{\mbox{$\frac{\partial {#1}}{\partial {#2}}$}}
\newcommand{\dt}{{\rm d}t}
\newcommand{\dx}{{\rm d}x}
\newcommand{\p}{\partial}
\newcommand{\pt}{\partial_t}
\newcommand{\ptt}{\partial^2_t}
\newcommand{\px}{\partial_x}
\newcommand{\pxx}{\partial^2_x}
\newcommand{\pp}{\partial{^2}}
\newcommand{\tr}{{\rm tr}\,}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%\DeclareMathOperator{\tr}{tr}
\newcommand{\rmA}{{\rm A}}
\newcommand{\rmB}{{\rm B}}
\newcommand{\rmC}{{\rm C}}
\newcommand{\rmD}{{\rm D}}
\newcommand{\rmE}{{\rm E}}
\newcommand{\rmF}{{\rm F}}
\newcommand{\rmG}{{\rm G}}
\newcommand{\rmH}{{\rm H}}
\newcommand{\rmI}{{\rm I}}
\newcommand{\rmJ}{{\rm J}}
\newcommand{\rmK}{{\rm K}}
\newcommand{\rmL}{{\rm L}}
\newcommand{\rmM}{{\rm M}}
\newcommand{\rmN}{{\rm N}}
\newcommand{\rmO}{{\rm O}}
\newcommand{\rmP}{{\rm P}}
\newcommand{\rmQ}{{\rm Q}}
\newcommand{\rmR}{{\rm R}}
\newcommand{\rmS}{{\rm S}}
\newcommand{\rmT}{{\rm T}}
\newcommand{\rmU}{{\rm U}}
\newcommand{\rmV}{{\rm V}}
\newcommand{\rmW}{{\rm W}}
\newcommand{\rmX}{{\rm X}}
\newcommand{\rmY}{{\rm Y}}
\newcommand{\rmZ}{{\rm Z}}
\newcommand{\rma}{{\rm a}}
\newcommand{\rmb}{{\rm b}}
\newcommand{\rmc}{{\rm c}}
\newcommand{\rmd}{{\rm d}}
\newcommand{\rme}{{\rm e}}
\newcommand{\rmf}{{\rm f}}
\newcommand{\rmg}{{\rm g}}
\newcommand{\rmh}{{\rm h}}
\newcommand{\rmi}{{\rm i}}
\newcommand{\rmj}{{\rm j}}
\newcommand{\rmk}{{\rm k}}
\newcommand{\rml}{{\rm l}}
\newcommand{\rmm}{{\rm m}}
\newcommand{\rmn}{{\rm n}}
\newcommand{\rmo}{{\rm o}}
\newcommand{\rmp}{{\rm p}}
\newcommand{\rmq}{{\rm q}}
\newcommand{\rmr}{{\rm r}}
\newcommand{\rms}{{\rm s}}
\newcommand{\rmt}{{\rm t}}
\newcommand{\rmu}{{\rm u}}
\newcommand{\rmv}{{\rm v}}
\newcommand{\rmw}{{\rm w}}
\newcommand{\rmx}{{\rm x}}
\newcommand{\rmy}{{\rm y}}
\newcommand{\rmz}{{\rm z}}
\newcommand{\BBA}{{\mathbb A}}
\newcommand{\BBB}{{\mathbb B}}
\newcommand{\BBC}{{\mathbb C}}
\newcommand{\BBD}{{\mathbb D}}
\newcommand{\BBE}{{\mathbb E}}
\newcommand{\BBF}{{\mathbb F}}
\newcommand{\BBG}{{\mathbb G}}
\newcommand{\BBH}{{\mathbb H}}
\newcommand{\BBI}{{\mathbb I}}
\newcommand{\BBJ}{{\mathbb J}}
\newcommand{\BBK}{{\mathbb K}}
\newcommand{\BBL}{{\mathbb L}}
\newcommand{\BBM}{{\mathbb M}}
\newcommand{\BBN}{{\mathbb N}}
\newcommand{\BBO}{{\mathbb O}}
\newcommand{\BBP}{{\mathbb P}}
\newcommand{\BBQ}{{\mathbb Q}}
\newcommand{\BBR}{{\mathbb R}}
\newcommand{\BBS}{{\mathbb S}}
\newcommand{\BBT}{{\mathbb T}}
\newcommand{\BBU}{{\mathbb U}}
\newcommand{\BBV}{{\mathbb V}}
\newcommand{\BBW}{{\mathbb W}}
\newcommand{\BBX}{{\mathbb X}}
\newcommand{\BBY}{{\mathbb Y}}
\newcommand{\BBZ}{{\mathbb Z}}

\newcommand{\real}{{\mathbb{R}}}
\newcommand{\comp}{{\mathbb{C}}}
\newcommand{\realR}{\mathbb{R}}

\newcommand{\SA}{{\mathcal A}}
\newcommand{\SB}{{\mathcal B}}
\newcommand{\SC}{{\mathcal C}}
\newcommand{\SD}{{\mathcal D}}
\newcommand{\SE}{{\mathcal E}}
\newcommand{\SF}{{\mathcal F}}
\newcommand{\SG}{{\mathcal G}}
\newcommand{\SH}{{\mathcal H}}
% \newcommand{\SI}{{\mathcal I}}
\newcommand{\SJ}{{\mathcal J}}
\newcommand{\SK}{{\mathcal K}}
\newcommand{\SL}{{\mathcal L}}
\newcommand{\SM}{{\mathcal M}}
\newcommand{\SN}{{\mathcal N}}
\newcommand{\SO}{{\mathcal O}}
\newcommand{\SP}{{\mathcal P}}
\newcommand{\SQ}{{\mathcal Q}}
\newcommand{\SR}{{\mathcal R}}
\newcommand{\SSS}{{\mathcal S}}
\newcommand{\ST}{{\mathcal T}}
\newcommand{\SU}{{\mathcal U}}
\newcommand{\SV}{{\mathcal V}}
\newcommand{\SW}{{\mathcal W}}
\newcommand{\SX}{{\mathcal X}}
\newcommand{\SY}{{\mathcal Y}}
\newcommand{\SZ}{{\mathcal Z}}
\newcommand{\BFA}{{\bf A}}
\newcommand{\BFB}{{\bf B}}
\newcommand{\BFC}{{\bf C}}
\newcommand{\BFD}{{\bf D}}
\newcommand{\BFE}{{\bf E}}
\newcommand{\BFF}{{\bf F}}
\newcommand{\BFG}{{\bf G}}
\newcommand{\BFH}{{\bf H}}
\newcommand{\BFI}{{\bf I}}
\newcommand{\BFJ}{{\bf J}}
\newcommand{\BFK}{{\bf K}}
\newcommand{\BFL}{{\bf L}}
\newcommand{\BFM}{{\bf M}}
\newcommand{\BFN}{{\bf N}}
\newcommand{\BFO}{{\bf O}}
\newcommand{\BFP}{{\bf P}}
\newcommand{\BFQ}{{\bf Q}}
\newcommand{\BFR}{{\bf R}}
\newcommand{\BFS}{{\bf S}}
\newcommand{\BFT}{{\bf T}}
\newcommand{\BFU}{{\bf U}}
\newcommand{\BFV}{{\bf V}}
\newcommand{\BFW}{{\bf W}}
\newcommand{\BFX}{{\bf X}}
\newcommand{\BFY}{{\bf Y}}
\newcommand{\BFZ}{{\bf Z}}
\def\bbR{\mbox{\bbfnt R}}
\newcommand{\vspaceAnkit}{\vspace{-3pt}}
\newcommand{\shiftq}{{\textbf{\textrm{q}}}}








% \newtheoremstyle{factindented}
%     {3pt}
%     {3pt}
%     {\addtolength{\leftskip}{1.5em}}
%     {}
%     {\bfseries}
%     {.}
%     {.5em}
%     {}
% %\theoremstyle{factindented}


% \newtheoremstyle{indented}
%     {3pt}
%     {3pt}
%     {\addtolength{\leftskip}{3em}}
%     {}
%     {\bfseries}
%     {.}
%     {.5em}
%     {}

% \theoremstyle{indented}







% \newcommand{\SCA}{{\mathscr{A}}}
% \newcommand{\SCB}{{\mathscr{B}}}
% \newcommand{\SCU}{{\mathscr{U}}}

\newcommand{\Star}{^{*}}

%\newcommand{\scM}{{\mathscr M}}
\newcommand{\scM}{{\mathcal M}}

\newcommand{\neweqline}{\ensuremath{\nn \\ &\quad }}

\newcommand{\framedot}[2]{\stackrel{{\rm #1}\bullet}{#2}}
\newcommand{\frameddot}[2]{\stackrel{{\rm #1}\bullet \bullet}{#2}}

\newcommand{\polar}[1]{\ensuremath{r_{#1}e^{\jmath \theta_{#1}}}}

\newcommand{\tarrow}[1]{\overset{\rightarrow}{#1}}

==> zzzDiscussions.tex <==

\clearpage 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Hi Jhon

Thanks!  I have a few questions.

You are optimizing J given by 45, right? yes

Is J a function of r? yes

What is the value of r*? it is 2 from t= [0,500] and then it is 4 
in Figure 1 did you mean to put r* in the legend? no that r is the output of the ESC

ok, but you could show r* as dotted right? yes


Is r* assumed to be UNknown to the controller? yes

back to 45.

Why is there +5?

I want to have a maximum value of 5 only, it can be any other value

are minimizing J(r)? maximizing

OK, let me edit 45, thank you Professor

are you ok with 45 now?

yes


ok, but something is confusing me.

In 45, if I take r = -1000000, I ccan make it huge! oh yess a quadratic term sorry

Is something missing??

please fix it thanks

my bad, a typo, already fixed

No problem!!!  thanks

ok so J(r*) = 5, right? yes  

and 5 is the maximum value, right? yes

good, so this is what I think we need to do next.

 

\begin{align}
    J(r)
        &=
            g(r - r^*) + 5;
    \label{eq:example_cost_function}
\end{align}

You chose

g(x) = -x^2, right?

yes just a quadratic funciton

ES does NOT know what g is and it does NOT know what r* is, right? correct

Great

you would like g(x) < 0 for all nonzero x, ok? ok


Please try a few g functions

g(x) = -|x|  can you do it? yes

g(x) = -|x-9|

g(x) = -x^2 -|x| yes

g(x) = -e^(-x^2) 

g(x) = -e^(-(x+4)^2)


can you please try these?  Thanks!

I will move this conversation to discussions 

ok

The exponential does not have a maximum

hmmmm let me think

I didnt want that sorry let me fix it


g(x) = e^(-x^2) - 1  How is this? yes that one will work


 

g(x) = e^(-(x+4)^2) - 1

good this is waht we need.  can you plese try these?  Thanks! yes


Great ttyl thanks!  email if any questions come up thanks! yes no problem thanks Professor, I will comment these lines, is that OK?
no need to since this is a scratch file  bye for now thanks!

ok, thanks Professor

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


here

Section 4------pls give the cost function for that section

J = -(r - r^*) + 5 ,

ok

Yes please start the section by stating the cost function thanks
to avoid confusion thats all




Section 5---------I am not sure what the plots show.  Is the main result that x is near 0?



you wrote J(x) but I think you mean J(r)

yes
 




this way we build up in complexity, ok?  Thanks 


 


Please read this:

Section 5---------what is CURRENTLy in setion 6-----OK AS IT IS NOW Thanks----is it clear?

this is not clear for me, do I maintain section 5?

ohhhhhhh you can delete the CURRENT section 5, sorry I got your question now

ok



In section 6, you have J(r) = -|x-9|.  Please relabel this section as section 5.  OK?

ok


Section 6--------this is a NEW section where you start with J(r) = -|x+2| and then at some point change J to J(r) = -|x-7|-----is it clear?




Current section 7:  replace r by r+2 and the at some point change to r-7



Current section 8----same idea---start with some r* and then at some point change to ANOTHER r*


This is basically the idea in showing that ES can find the NEW optimal point

Does that make sense?

yes


One more thing.  This might be a little tricky but it is the kind of thing we like to do.  Here goes:

Plot J(r) in a light colored line.

At each point in time (iteration k) plot a dot ON the plot of J(r) which corresponds to the CURRENT value of J(r_k)

Do you sort of see what I mean?

yes that is what I sort wanted to do in Figure 4 but if I only plot the points we are not going to see how those points evolve 

right, so I need to tell you what to do next.  This idea if from Juan:

So you have a sequence of points J(r1), J(r2), ....

right?

yes

so so as you plot J(rk), and k increases, then you change the color from yellow to blue-----in other words, you use "heat" to indicate time!

Juan did this in a paper, I will  send it to you ok?  Thanks

ok

Thanks.  Any questions?

in the cases where the optimal value changes from -2 to 7, we will have 2 differet cost functions 

Right.  At the instant that J changes, just start a NEW plot, thats all.


ok

anything else?


no, thank you

ok, I will send you Juans paper.

did you get my calendar invitation?

yes I get your calendar shared with me but not an invitation to meet but I will be there on thursday 

just arrive at noon Thursday thanks


great.  Please also send me a calendar invitation thanks.

ok thank you

great ttyl thanks!



%%%%
Aidan: 

Each of the cost function sections are the ones that I have done for all 3 of the oscillator, unstable oscillator, and double integrator. 

Note that the cost function in section VIII is written in terms of optical parameters, I can change this if needed.

Do we want to include examples of rstar changing from one value to another?
 
What are the rules for plots? 
Grid always on?
12 pt Times New Roman font for axes? 
Legend in any particular spot? 

Could also increase Rdu to get rid of bang-bang behavior in the U-plot. 

Thanks.
%%%%
Hi Aidan for the Cost function Plots I believe it is easier if you send me your code and I integrate it with mine, I already have that code ready, so send me the code for the 3 examples please when they are ready. 

Thanks a lot.

Jhon
%%%%%

Aidan: Sent email!

Thank you got it.



DDDDDDDD  Thanks for the update



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Hi Jhon

Please add authors

yes, sure

When do you plan to add the examples?

Hi Professor, I am doing so today

ok, thanks, I will check back later

I may do a little editing of the introduction  Did you paste it from another paper?

yes please Professor. 

No I mix the PCAC intro that jacob paste on the paper with an intro of the ESC paper that I presented in Scitech this year to introduce the problem so it is built from that, not copied.


ok, thanks, I will edit it no problem thanks

We will meet tomorrow at noon thanks

Thank you Professor, yes sure.


%%%%%%%%%%%%%%

Hi Professor. The plots of the undamped mass-pring system is already in the examples section. Maybe we can interate over them and discuss the changes for the double integrator example?


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

here

sorry I wanted to make a few changes

no problem professor
how are you doing?


All good I havent emailed you yet but the three examples are here, the double integrator has a disturbance as well. The only thing I am thinking of is changing the r_star of one of the examples

GOOD!  what is the disturbance signal????  Jhon, what disturbance signal did you choose?

Constant disturbance in the input

ok, so essentially a control-input bias.  Please say that


yes

ok, let me finish editing the oscillator example and then you can check it.  once you agree it is ok, then you can edit the others.  Please follow me

ok, thank you

I will finish editing the oscillator example.  Then I would like you to copy my edits as carefully as you can for the other 2 examples, ok?  Thanks


ok Professor




here


are (1)--(5) those totally standard equations?



what do you mean standard equations?

I mean, would I find (1)--(5) in books and paper by krstic?



no, not at all, krstic does everything continuous, and not demodulation, in fact his paper only uses a low pass filter and high pass filter in continuous time, but the gain 2/a_es is needed, as proved in a paper by ying tan and nesic.


ok I have a few qustions

In (1)------why do you have a minus sign instead of (1-omega_h Ts)?


because of the result of the transfer function in figure 2. the relation between y_h,k and J_k is z-1/(z + whT_s - 1)

ok, but you COULD remove the minus sign and write (1-omega_h Ts), right?



yes, I just follow the block diagram but yes, and I can change it as well


in (2), are you modulating yk to get yd?


I am demodulating actually, when m

then why not put yh at the END of the equation?



y_h?
yes y_h,k at the END of the line?




ohh I see, ok yes


ok, then write it like this:

yd,k = \frac{2bes omegalTs}{aes}sin(xxx)y_h,k


ok
is it clear?


yes, also changing the sign of (whTs-1) in 1?


yes

now you often write:

omega*k*Ts

but it is more natureal to write

k*omega*Ts

oik?




ok Professor

let me check one sec.......

follow me





ok

are you still here?


yes

do you know how to follow my cursor?pls follow me


yes ok


ok, thanks.  I dont think I can make any more improvements now.  But we did clean up a few things

I think this algorithm has way too much notation-----there are a huge number of variatbles, like gamma_a and gamma_K, things like that.  I am sure there is a way to vastly clean this up

I agree. I can make a presentation on that and lets clean it up. I agree


You have an algorithm for adjusting ES, but it involves many parameters that the user must choose.  I would like to find a way to streamline and simplify this----yes you got it to work, but it just seems quite involved


yes. Let me also show you the other one that I have after submission

ok, lets not worry about thisnow

lets finish up this paper.  Then you will work with Ethan, right?  and also we will use ES for the paper with Aidan, right?



yes, yes.

Regarding the y notation, do I keep it? or Do I change it to another one?

keep it.  Too complicated to change it

follow me.......










